Enabling Design Space Exploration of DRAM Caches in Emerging Memory Systems

The increasing growth of applications' memory capacity and performance demands has led the CPU vendors to deploy heterogeneous memory systems either within a single system or via disaggregation. For instance, systems like Intel's Knights Landing and Sapphire Rapids can be configured to use high bandwidth memory as a cache to main memory. While there is significant research investigating the designs of DRAM caches, there has been little research investigating DRAM caches from a full system point of view, because there is not a suitable model available to the community to accurately study largescale systems with DRAM caches at a cycle-level. In this work we describe a new cycle-level DRAM cache model in the gem5 simulator which can be used for heterogeneous and disaggregated systems. We believe this model enables the community to perform a design space exploration for future generation of memory systems supporting DRAM caches.

==> background.tex <==
\section{Background}
\label{sec:background}

\subsection{Background on heterogeneous and disaggregated memory systems}

With the growing footprint of large scale applications, commercial products have been emerging in the market
to accommodate the memory requirements of the today's demanding workloads. Intel introduced Optane Data-Center
Persistent-Memory-Modules (NVRAM) and as a replacement for conventional DRAMs~\cite{hildebrand2021case}. Even though NVRAM provides much larger capacity than DRAM, it has 3x longer latency and
60\% lower bandwidth than DRAM ~\cite{izraelevitz2019basic}. Hardware caching through DRAM DIMMs, has been employed in Intel's
Cascade Lake product to hide the long latency of NVRAM. Intel has announced the release of the new generation of Xeon processor called Sapphire Rapid~\cite{sapphire}
which includes an HBM2 device capable of caching for DDR5 memory.

Memory interface/interconnect technologies like CXL~\cite{van2019hoti} enable disaggregated memory systems to utilize
available memory resources better~\cite{calciu2021rethinking,wahlgren2022evaluating}. CXL is reported to be included in Intel's Sapphire Rapids. Moreover, CXL is
anticipated to be highly employed in cloud servers where ...\Maryam{needs be completed}.
Directly attached memories can be a cache to a large (remote/disaggregated) memory pool
(connected via interconnects like CXL~\cite{van2019hoti}).
Our model allows to study such DRAM cache topologies. \Maryam{needs be completed}.

\subsection{Background on \gem{}'s memory subsystem}\Maryam{if needed space, shorten this part}

The \gem{} simulator is based on an event-driven full-system simulation engine.
It supports models of many system components, including a memory controller, a detailed DRAM model, an NVM model, and a model for different CPUs, caches, and others.
The memory controller module added to \gem{} by Hansson et al.~\cite{hansson2014simulating} focuses on modeling the state transitions of the memory bus and the memory banks.
While it is not ``cycle accurate'', it is \emph{cycle level}, and the memory controller is designed to enable fast and accurate memory system exploration.

The memory controller in \gem{} was refactored in ~\cite{gem5-workshop-presentation} where two components were defined to simulate a real memory controller.
(1) The \textit{memory controller} receives commands from the CPU and enqueues them into appropriate queues and manages their scheduling to the memory device.
(2) The \textit{memory interface} deals with device/media-specific timings, manages the device-specific operations and communicates with the memory controller.

Moreover, the most recent release of \gem{} further improves the flexibility and modularity of memory controller and interfaces~\cite{akram2022modeling}.
Most importantly, it provides support for HBM2 interface and memory controller, where each physical channel is consisted of
two pseudo-channels with peak theoretical bandwidth of 32 GB/s per channel.
The DRAM cache model presented in this work can employ any of these memory controller and interfaces of \gem{} without any modifications.
Like \gem's current memory controller, our DRAM cache model's goal is for cycle-level simulation to enable micro-architectural exploration and flexibility, not cycle-by-cycle accuracy to a single design.


==> validation.tex <==
\section{Validation}
\label{sec:validation}

\begin{comment}
How to show that the model is working correctly (in terms of functionality as well as performance modeling)?
\begin{itemize}
\item Rely on traffic generator baseline studies (with read only hits, read only misses kind of patterns), and show that we get expected results
\item Comparison of performance between the model and Intel Cascade lake results (will be difficult to do in full-form, but we might be able to think of some related experiments to present the point)
\end{itemize}
\end{comment}

In this section, we present the validation of our DRAM cache model in \gem.
Any simulation model needs to be functionally correct, as well as provide accurate performance statistics.
To ensure functional validation,
% We performed following actions for the functional validation of the implemented model:
%\item We successfully ran a collection of benchmarks\footnote{Bubblesort, Dhrystone, FloatMM, IntMM, miniAMR, miniGMG, Oscar, Perm, Quicksort, RealMM, RSBench, Towers, %Treesort, XSBench} in the \textit{SE (system call emulation)} mode of \gem~and compared the output of these benchmarks with the reference output.
% \begin{itemize}
we successfully performed Linux kernel boot tests in \gem{} full system mode, and
we ran some commonly used HPC class benchmarks in \gem{} full-system mode, which are presented in Section~\ref{sec:realBench} of this paper.

The evaluation of the accuracy of the performance model is generally not straightforward. Still, reasonable confidence can be established in the performance model by relying on the evaluation of performance numbers in controlled experiments.
We performed a comparison of the effective memory bandwidth observed with \gem's default memory controller (\textit{DMC}) and the unified DRAM cache controller (\textit{UDCC}).
We rely on a synthetic read memory traffic pattern such that (nearly) \textit{all requests will be hits in the DRAM cache} in the case of a system where we use \textit{UDCC}.
We use both a linear and a random traffic pattern.
Figure~\ref{fig:valid} provides both controllers' read bandwidth and compares these numbers to the theoretical peak bandwidth possible with the DDR4 device used in this experiment.
As expected, we observe that the bandwidth attained by \textit{DMC} and \textit{UDCC} is very close.
The scheduling policy implemented in both controllers (details in Section~\ref{sec:sched}) can explain the slight difference.
The effective bandwidth in both cases is less than the theoretical peak bandwidth.

The access amplification (total number of memory accesses divided by the demand requests) can be significant in DRAM caches, especially in the case of writes.
We compare the access amplification of our model with that of the actual hardware.
We use the access amplification numbers presented by Hildebrand et al.~\cite{hildebrand2021case} on an Intel Cascade Lake system.
We calculate the access amplification values for \textit{UDCC} by dividing the effective bandwidth (seen by the LLC) by the sum of the average bandwidth of DRAM and NVRAM devices for a particular run.
The comparison of the two access amplification values is shown in Figure~\ref{fig:valid2}.
Our results match the actual hardware in all cases with only one exception.
The reason for smaller access amplification for write misses is that our implementation slightly optimizes the write requests.
In actual hardware, on a write miss in DRAM cache, the block is first allocated by reading it from NVRAM and then writing it into DRAM. The actual data is then written into the DRAM. We merge these two DRAM writes, and thus, our implementation leads to one less access for a write miss compared to the actual hardware.

Finally, we manually stepped through the operations of different kinds of accesses (reads/writes and hits/misses) to ensure they behaved as expected.

\begin{figure}
  \centering
  \includegraphics[scale=0.5]{figures/bwcomp.pdf}
  \vspace{-1ex}
  \caption{Read bandwidth comparison between \gem~default memory controller (\textit{DMC}), unified DRAM cache controller (\textit{UDCC}), and the theoretical peak bandwidth on DDR4. In case of \textit{UDCC}, all accesses hit in the DRAM cache. Two different traffic patterns (linear, random) are used. Read buffer size in \textit{MC}, and \textit{ORB} size in \textit{UDCC} is 256 entries.}
  \label{fig:valid}
\end{figure}

 \begin{figure}
  \centering
  \includegraphics[scale=0.5]{figures/accAmpl.pdf}
  \vspace{-1ex}
  \caption{Access amplification observed with \textit{UDCC} in \gem{} and on the real hardware (Hildebrand et al.~\cite{hildebrand2021case}).}
  \label{fig:valid2}
\end{figure}

